Causal Identification under Markov Equivalence

Assessing the magnitude of cause-and-effect relations is one of the central challenges found throughout the empirical sciences. The problem of identification of causal effects is concerned with determining whether a causal effect can be computed from a combination of observational data and substantive knowledge about the domain under investigation, which is formally expressed in the form of a causal graph. In many practical settings, however, the knowledge available for the researcher is not strong enough so as to specify a unique causal graph. Another line of investigation attempts to use observational data to learn a qualitative description of the domain called a Markov equivalence class, which is the collection of causal graphs that share the same set of observed features. In this paper, we marry both approaches and study the problem of causal identification from an equivalence class, represented by a partial ancestral graph (PAG). We start by deriving a set of graphical properties of PAGs that are carried over to its induced subgraphs. We then develop an algorithm to compute the effect of an arbitrary set of variables on an arbitrary outcome set. We show that the algorithm is strictly more powerful than the current state of the art found in the literature.

==> defs.tex <==
\begin{defn}[Definite Status Node]
A non-endpoint node $X$ along a path is called a \textit{definite collider} (DC) if both incident edges are into $X$.
A non-endpoint node $X$ along a path is called a \textit{definite non-collider} (DNC) if one of the incident edges is out of $X$ or it is $A*\!\!\--\!\!\circ X \circ\!\!\--\!\!*B$ such that $A$ and $B$ are not adjacent.
\end{defn}

\begin{defn}[Definite Status Path]
A path is of definite status if every non-endpoint node along the path is of definite status.
\end{defn}

%\begin{defn}[Proper Path]
%Given two sets of nodes $\mathbf{X}$ and $\mathbf{Y}$, a path between them is called \textit{proper} if one of the endpoints is in $\mathbf{X}$ and the other is in $\mathbf{Y}$, and no other node on the path is in $\mathbf{X}$ or $\mathbf{Y}$.
%\end{defn}

\begin{defn}[Discriminating Path]
Given a MAG $\mathcal{M}$ or a PAG $\mathcal{P}$, a path between $D$ and $C$, $u=\langle D,\dots ,A,B,C\rangle$, is said to be a discriminating path for $B$ if:
\begin{enumerate}
\item $u$ includes at least three edges.
\item $B$ is a non-endpoint node along the path, and is adjacent to $C$ on $u$.
\item $D$ is not adjacent to $C$, and every node between $D$ and $B$ is a (definite) collider on $u$ and is a parent of $C$.
\end{enumerate}
\end{defn}

==> proofs.tex <==
\subsection{Proposition~\ref{prop:pccompsubpag}}

\begin{proof}[Proof of Proposition~\ref{prop:pccompsubpag}]
If $X$ and $Y$ are in the same c-component in $\mathcal{D}_\mathbf{A}$, then there is a path $p$ in $\mathcal{D}_\mathbf{A}$ composed of nodes $\langle X=V_0,\dots,Y=V_m\rangle$, $m\geq 1$, such that $V_i\in\mathbf{A}$ and $V_i\leftarrow L_{i,i+1}\rightarrow V_{i+1}$, $0\leq i<m$.

By lemma~\ref{lem:dagmag}, $X$ and $Y$ are in the same pc-component in $\mathcal{M}$, the MAG of $\mathcal{D}$ over $\mathbf{V}$, due to a path $p'$ over a subsequence of $p$.
Also, by lemma~\ref{lem:magpag}, $X$ and $Y$ are in the same pc-component in $\mathcal{P}$, the PAG of $\mathcal{M}$, due to a path $p^*$ over a subsequence of $p'$.
Since all the nodes along $p^*$ are in $\mathbf{A}$, then $p^*$ is present in $\mathcal{P}_\mathbf{A}$, hence $X$ and $Y$ are in the same pc-component in $\mathcal{P}_\mathbf{A}$.
\end{proof}

\begin{lemma}
\label{lem:dagmag}
Let $\mathcal{G}(\mathbf{V},\mathbf{L})$ be a DAG, and $\mathcal{M}$ be the MAG over $\mathbf{V}$ that represents the DAG.
For any $X,Y\in\mathbf{V}$, if there is a bi-directed path $p$ between $X$ and $Y$ in $\mathcal{G}$, then there is a path $p'$ between $X$ and $Y$ in $\mathcal{M}$ over a subsequence of $p$ such that (1) all the non-endpoint nodes are colliders, and (2) all directed edges on $p'$ are not visible.
\end{lemma}

\begin{proof}
We prove this lemma by induction on the size (number of bi-directed edges) of the bi-directed path between $X$ and $Y$ in $\mathcal{G}$. 
Before we start with the proof, note that the only possible directed edges along the path $p'$ are the first and last edges since all non-endpoint nodes are colliders.  Also, we will prove the following stronger statement in order to prove our main lemma.

\begin{quote}
Let $\mathcal{G}(\mathbf{V},\mathbf{L})$ be a DAG, and $\mathcal{M}$ be the corresponding MAG over $\mathbf{V}$. For any $X,Y\in\mathbf{V}$, if there is a bi-directed path $p$ between $X$ and $Y$ in $\mathcal{G}$, then there is a path $p'$ between $X$ and $Y$ over a subsequence of $p$ in $\mathcal{M}$ such that:
\begin{enumerate}
\item all the non-endpoint nodes are colliders; and 
\item all directed edges $A\rightarrow B$ on $p'$, have an inducing path between $A$ and $B$ into $A$ in $\mathcal{G}$.
\end{enumerate}
\end{quote}

The above statement implies the main lemma as the only difference is the second point regarding the directed edges along path $p'$ in $\mathcal{M}$. It is evident that a directed edge in MAG $\mathcal{M}$ is not visible if it has an inducing path into its source in DAG $\mathcal{G}$ where $\mathcal{G}$ is in the equivalence class of $\mathcal{M}$.

Consider as a base case path $p$ of size 1 between $X$ and $Y$ in $\mathcal{G}$. 
The bi-directed edge between $X$ and $Y$ ($X\leftarrow L_{XY}\rightarrow Y$) is an inducing path between $X$ and $Y$ relative to the latent variable $L_{XY}$ in $\mathcal{G}$. Hence, $X$ and $Y$ are adjacent in MAG $\mathcal{M}$. If neither $X$ nor $Y$ is an ancestor of the other in $\mathcal{G}$, then the edge between $X$ and $Y$ in $\mathcal{M}$ is bi-directed and the lemma holds. If $X$ is an ancestor of $Y$ or the opposite in $\mathcal{G}$, then the edge in $\mathcal{M}$ is directed ($X\rightarrow Y$ or $X \leftarrow Y$). 
In both cases, the latent variable $L_{XY}$ in $\mathcal{G}$ provides an inducing path between $X$ and $Y$ that is into both ends. 
Hence, the lemma holds.

In the induction step, we assume that the lemma holds for bi-directed paths between $X$ and $Y$ in $\mathcal{G}$ of length $\leq n$ and prove it for bi-directed paths of length $n+1$.
Consider the bi-directed path $p=\langle X,O_1,\dots,O_n,Y\rangle$ of length n+1 in $\mathcal{G}$. 
We split the path into two paths $p_1=\langle X,O_1\rangle$ and $p_2=\langle O_1,\dots,Y\rangle$.
By the assumption of the induction step, the lemma holds for each path and there are collider paths $p_1'$ and $p_2'$ in MAG $\mathcal{M}$ corresponding to $p_1$ and $p_2$ in $\mathcal{G}$.
Consider the options of path $p_1'$:
\begin{enumerate}
\item[case 1:] $O_1$ is not an ancestor of $X$ in $\mathcal{G}$. Hence, the edge between $X$ and $O_1$ in $\mathcal{M}$ is into $O_1$ ($X\rightarrow O_1$ or $X\leftrightarrow O_1$). If the edge is directed ($X\rightarrow O_1$), there is an inducing path into $X$ in $\mathcal{G}$ ($X\leftarrow L_{XO_1}\rightarrow O_1$). Now consider the first edge in $p_2'$ which, according to the lemma, could be one of the following two options:
\begin{enumerate}
\item[case 1-1:] The edge is $O_1\leftrightarrow O_i$. Then, edge $X\rightarrow O_1$ concatenated with path $p_2'$ create a path between $X$ and $Y$ in $\mathcal{M}$ which is consistent with the conditions in the lemma. Hence, the lemma holds.

\item[case 1-2:] The edge is $O_1\rightarrow O_i$.
By the induction step, there is an inducing path between $O_1$ and $O_i$ into $O_1$ in $\mathcal{G}$ so the edge $O_1\rightarrow O_i$ is not visible in $\mathcal{M}$. Hence, $X$ and $O_i$ must be adjacent in $\mathcal{M}$ for otherwise edge $O_1\rightarrow O_i$ would be visible.
Also, the edge between $X$ and $O_i$ is directed into $O_i$, otherwise the MAG is not ancestral.
Moreover, there is an inducing path between $X$ and $O_1$ that is into $X$ and there is an inducing path between $O_1$ and $O_i$ that is into $O_1$.
Node $O_1$ is a collider between those two inducing paths and an ancestor of $O_i$.
So, there is an inducing path between $X$ and $O_i$ that is into $X$ in $\mathcal{G}$.
Hence, there is a path between $X$ and $Y$ in $\mathcal{M}$ composed of edge $X\rightarrow O_i$ and the subpath of $p_2'$ $\langle O_i,\dots,Y\rangle$ which is consistent with the conditions of the lemma. 
\end{enumerate}

\item[case 2:] $O_1$ is an ancestor of $X$ in $\mathcal{G}$. Hence, the edge between $X$ and $O_1$ in $\mathcal{M}$ is $X\leftarrow O_1$. 
Also, there is an inducing path between $X$ and $O_1$ into $O_1$ in $\mathcal{G}$ ($X\leftarrow L_{XO_1}\rightarrow O_1$) so edge $X\leftarrow O_1$ in $\mathcal{M}$ is not visible. Next, we consider the first edge in path $p_2'$.

\begin{enumerate}
\item[case 2-1:] The edge is $O_1\leftrightarrow O_i$. Then, path $p_2'$ is a collider path into $O_1$ in $\mathcal{M}$.
We show, by induction, that $X$ is a child of each node along $p_2'$ in $\mathcal{M}$ starting from $O_1$ until there exist a bi-directed edge between $X$ and some node along $p_2'$.
For the base case, $O_i$ is adjacent to $X$ for otherwise edge $X\leftarrow O_1$ is visible.
Also, the edge is into $X$, otherwise the MAG is not ancestral.
If the edge is bi-directed, then we are done and the statement holds, otherwise the edge is out of $O_i$.
In the induction step, assume all nodes along path $p_2'$ starting with $O_i$ until $O_j$ are parents of $X$.
We have a collider path between $O_{j+1}$, which could be $Y$, and $O_1$ that is into $O_1$ and each collider is a parent of $X$. Hence, node $O_{j+1}$ must be adjacent to $X$ for otherwise $X\leftarrow O_1$ is visible.
Also, the edge between $X$ and $O_{j+1}$ is into $X$ for otherwise $\mathcal{M}$ is not ancestral due to $O_j\rightarrow X \rightarrow O_{j+1}$ and $O_{j+1}*\!\!\rightarrow O_j$.
Hence, the statement holds.

If there exist a bi-directed edge between $X$ and some node $O_k$ along $p_2'$, then there exist a path between $X$ and $Y$ composed of $X\leftrightarrow O_k$ and the subpath of $p_2'$ $\langle O_k,\dots,Y\rangle$ that is consistent with the lemma. Otherwise, $X$ and $Y$ are adjacent and $Y$ is a parent of $X$ by the above induction.
In the latter case, consider the concatenated path of $p_1'$ and $p_2'$ ($X\leftarrow O_1 \leftrightarrow O_i \xdashleftrightarrow{\hspace{3em}} O_j \leftarrow\!\!\!* Y$). There exist an inducing path between every two consecutive nodes and every non-endpoint node is an ancestor of $X$. Also, by the induction assumption, the first and last edges along the path have inducing paths into the source node ($O_1$, and $Y$ if $O_j\leftarrow Y$).
Hence, there exist an inducing path between $X$ and $Y$ that is into $Y$ in $\mathcal{G}$ and the lemma holds.

\item[case 2-2:] The edge is $O_1\rightarrow O_i$.
Both edges $X\leftarrow O_1$ and $O_1\rightarrow O_i$ have inducing paths into $O_1$ in $\mathcal{G}$ by the induction assumption. Hence, $X$ and $O_i$ are adjacent in $\mathcal{M}$. We consider all the orientations of the edge between $X$ and $O_i$ in $\mathcal{M}$. 
If the edge is bi-directed, then there is a path between $X$ and $Y$ in $\mathcal{M}$ composed of $X\leftrightarrow O_i$ and the subpath of $p_2'$ $\langle O_i,\dots,Y\rangle$ consistent with the conditions of the lemma.
If the edge is out of $X$, then we have the path $\langle X,O_i,\dots,Y\rangle$. Moreover, the edge $X\rightarrow O_i$ has an inducing path into $X$ in $\mathcal{G}$. The reason is that $O_1$ is a collider in $\mathcal{G}$ between the two inducing paths corresponding to edges $X\leftarrow O_1$ and $O_1\rightarrow O_i$ and the node is an ancestor of $X$ and $O_i$. Hence, the lemma holds too.
The last case is when the edge is out of $O_i$, hence we have the path $X\leftarrow O_i,\dots,Y$. Similar to the earlier case, the edge $X\leftarrow O_i$ has an inducing path into $O_i$ in $\mathcal{G}$. The argument for this case follows same as that of case 2-1.
\end{enumerate}
\end{enumerate}
This exhausts all the options in the induction step and the lemma holds.
\end{proof}

\begin{lemma}
\label{lem:magpag}
Let $\mathcal{M}$ be a MAG over $\mathbf{V}$, and $\mathcal{P}$ be the PAG that represents the equivalence class of $\mathcal{M}$.
For any $X,Y\in\mathbf{V}$, if there is a path $p$ between $X$ and $Y$ in $\mathcal{M}$ such that (1) all non-endpoint nodes are colliders and (2) all directed edges, if any, are not visible, 
then there is a path $p^*$ between $X$ and $Y$ in $\mathcal{P}$ over a subsequence of $p$ such that (1) all non-endpoint nodes along the path are definite colliders, and (2) none of the edges are visible.
\end{lemma}

\begin{proof}
We use the following lemma from \citep[pp. 208]{zhang2006causal} several times throughout the proof.

\begin{quote}[\textbf{Lemma I}: ]
If a path $\langle U,\dots, X,Y,Z\rangle$ is a discriminating path for $Y$ in $\mathcal{M}$, and the corresponding subpath between $U$ and $Y$ in $\mathcal{P}$ is (also) a collider path, then the path is also a discriminating path for $Y$ in $\mathcal{P}$.
\end{quote}

%\paragraph*{\textbf{lemma I:}} If a path $\langle U,\dots, X,Y,Z\rangle$ is a discriminating path for $Y$ in $\mathcal{M}$, and the corresponding subpath between $U$ and $Y$ in $\mathcal{P}$ is (also) a collider path, then the path is also a discriminating path for $Y$ in $\mathcal{P}$.

%\paragraph{}
%We denote the sequence of nodes along a path between $X$ and $Y$ by $\langle X=O_0,\dots,O_n=Y\rangle$.
In order to prove the main lemma, we start with a simpler lemma.

\begin{quote}[\textbf{lemma II}: ]
For any $X,Y\in\mathbf{V}$, if $X$ and $Y$ are not adjacent and there is a collider path between $X$ and $Y$ in $\mathcal{M}$, denoted $p=\langle X=O_0,\dots,O_n=Y\rangle$, and $p$ is the shortest collider path between $X$ and $Y$ over any subsequence of $O_1,\dots,O_{n-1}$ in $\mathcal{M}$, then path $p$ is of definite status in $\mathcal{P}$.
%, i.e. all non-endpoint nodes along the path are colliders ($\rightarrow O_i\leftarrow$) or non-colliders ($\leftarrow O_i *\!\!\--\!\!*$, or $\circ\!\!\--\!\!\circ O_i$).
\end{quote}

%\paragraph*{\textbf{lemma II:}}
%For any $X,Y\in\mathbf{V}$, if $X$ and $Y$ are not adjacent and there is a collider path $p$ between $X$ and $Y$ in $\mathcal{M}$ and $p$ is the shortest collider path between $X$ and $Y$ over any subsequence of $O_1,\dots,O_{n-1}$ in $\mathcal{M}$, then path $p$ is of definite status in $\mathcal{P}$.

\paragraph*{proof:}
We prove this lemma by contradiction.
For that purpose, we first establish the following claim.

\begin{quote}[\textbf{claim$_{II}$}: ]
For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p$ in PAG $\mathcal{P}$, then $O_{j+1}$ is a parent of $O_{j-1}$ in $\mathcal{M}$.
\end{quote}

%\tab \textbf{claim$_{II}$:} For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p$ in PAG $\mathcal{P}$, then $O_{j+1}$ is a parent of $O_{j-1}$ in $\mathcal{M}$.

The claim holds if all the non-endpoint nodes are of definite status.
However, suppose there exist at least one non-endpoint node that is not of definite status.
We prove the claim by induction.
In the base case, let $O_j$ where $1\leq j\leq n-1$ be the first non-definite status node along $p$ that is closest to $X$.
Then, nodes $O_{j-1}$ and $O_{j+1}$ must be adjacent for otherwise we are able to detect the collider at $O_j$.
The edge between $O_{j-1}$ and $O_{j+1}$ can't be bi-directed in $\mathcal{M}$ since this creates a shorter collider path over a subsequence of $O_1,\dots,O_{n-1}$ and violates our choice of path $p$ in lemma II.
Suppose $O_{j-1}$ is a parent of $O_{j+1}$ in $\mathcal{M}$.
The collider path between $X$ and $O_j$ is of definite status in $\mathcal{P}$ as $O_j$ is the first node that is not of definite status along the path.
If $O_{j-2}$ is not adjacent to $O_{j+1}$ then $\langle O_{j-2},O_{j-1},O_{j},O_{j+1}\rangle$ is a discriminating path for $O_j$ in $\mathcal{M}$ and the subpath $\langle O_{j-2},O_{j-1},O_{j}\rangle$ is a collider path in $\mathcal{P}$.
Hence, $O_j$ is oriented as a collider along the path in $\mathcal{P}$ by lemma I and that contradicts our choice of $O_j$ which is not of definite status.
Hence, $O_{j-2}$ is adjacent to $O_{j+1}$ and the edge is out of $O_{j-2}$.
If the edge is bi-directed, we violate our choice of $p$ in lemma II as shortest over $O_1,\dots,O_{n-1}$ and if the edge is out of $O_{j+1}$, we violate the ancestral property in $\mathcal{M}$.
We apply the previous argument by induction on all the nodes starting with $O_{j-2}$ back to $O_0$.
Hence, each node $O_k$ where $0\leq k\leq j-1$ is adjacent to $O_{j+1}$ and the edge is out of $O_k$ in $\mathcal{M}$.
Now, $X$ has an edge out of it and into $O_{j+1}$ which violates our choice of $p$ in lemma II as the shortest path.
Therefore, the initial assumption about the orientation of the edge between $O_{j-1}$ and $O_{j+1}$ is invalid and the edge is out of $O_{j+1}$ in $\mathcal{M}$.

In the induction step, we assume that the lemma holds for some non-definite status node $O_r$ where $1\leq r\leq n-1$ and we prove that the lemma holds for the next non-definite status node $O_{r+l}$ along the path.
Similar to the base case argument, the nodes $O_{r+l-1}$ and $O_{r+l+1}$ must be adjacent and the edge can't be bi-directed in $\mathcal{M}$.
Assume that the edge is out of $O_{r+l-1}$ in $\mathcal{M}$, then we show by induction, similar to the base case, that each node $O_j$ where $r\leq j\leq r+l-1$ is adjacent to $O_{r+l+1}$ and the edge is out of $O_j$.
Now, we consider node $O_r$ which is not of definite status and note that $O_{r+1}$ is a parent of $O_{r-1}$ in $\mathcal{M}$ by the induction step.
We use the same argument by induction as before to show that each node $O_k$ where $r+1\leq k\leq r+l$ is adjacent to $O_{r-1}$ and the edge is out of $O_k$.
This creates an inducing path between $O_{r-1}$ and $O_{r+l+1}$ hence those two nodes must be adjacent in $\mathcal{M}$, otherwise we violate the maximality property.
The edge between $O_{r-1}$ and $O_{r+l+1}$ can't be bi-directed in $\mathcal{M}$ as it violates the choice of the path in lemma II.
If the edge is out of $O_{r-1}$, then we violate the ancestral property of $\mathcal{M}$ due to the structure $O_{r+l}\rightarrow O_{r-1} \rightarrow O_{r+l+1}$ and $O_{r+l}\leftarrow\!\!*O_{r+l+1}$.
Similarly, the edge can't be out of $O_{r+l+1}$.
Hence, the initial assumption that the edge between $O_{r+l-1}$ and $O_{r+l+1}$ is out of $O_{r+l-1}$ is invalid and the edge is out of $O_{r+l+1}$ in $\mathcal{M}$.
Hence , the claim holds for $O_{r+l}$.

With the previous claim proven, we finish our proof for lemma II by establishing the following claim.

\begin{quote}[\textbf{claim$_{II}^*$}: ]
For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p$ in $\mathcal{P}$, then $O_{j-1}$ is a parent of $O_{j+1}$ in $\mathcal{M}$.
\end{quote}
%\tab \textbf{claim$_{II}^*$:} For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p$ in $\mathcal{P}$, then $O_{j-1}$ is a parent of $O_{j+1}$ in $\mathcal{M}$.

\textbf{claim$_{II}^*$} is symmetric to \textbf{claim$_{II}$}.
Hence, its proof is carried out same as the proof of the previous claim with the difference of starting with the first non-definite status node that is closest to $Y(O_n)$ instead of $X(O_0)$.
However, both claims being valid is contradicting as long as there exist at least one non-definite status node $O_j$ where $1\leq j\leq n-1$.
Therefore, all the nodes along path $p$ are of definite status.
This concludes our proof of lemma II.

Now, we are ready to prove our main lemma.
We choose the shortest subsequence of $p$ between $X$ and $Y$ in $\mathcal{M}$, denoted $p^*$, such that (1) all none endpoint nodes along the path are colliders, and (2) none of the directed edges, possibly the first and last edges along $p^*$, are visible.
We show that path $p^*$ is of definite status and none of the directed edges along the path are visible in $\mathcal{P}$.

If $p^*$ is a single edge between $X$ and $Y$, then the edge is not visible in $\mathcal{M}$ and hence it is not visible in $\mathcal{P}$ and the lemma holds.
Otherwise, path $p^*$ is a collider path with at least one non-endpoint node.
It is evident that if the first or last edge along $p^*$ is directed and not visible in $\mathcal{M}$, then those edges will not be visible in $\mathcal{P}$ if directed.
We use a proof similar to that of lemma II to prove that $p^*$ is of definite status in $\mathcal{P}$ and start with the following claim.

\begin{quote}[\textbf{claim$_I$}: ]
For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p^*$ in $\mathcal{P}$, then $O_{j+1}$ is a parent of $O_{j-1}$ in $\mathcal{M}$.
\end{quote}

%\tab \textbf{claim$_I$:} For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p^*$ in $\mathcal{P}$, then $O_{j+1}$ is a parent of $O_{j-1}$ in $\mathcal{M}$.

We prove this claim by induction.
In the base case, we choose the first node $O_j$ that is not of definite status along the path in $\mathcal{P}$ and closest to $X$.
$O_{j-1}$ and $O_{j+1}$ are adjacent in $\mathcal{M}$ and the edge can't be bi-directed because of the choice of $p^*$.
First, we assume that the edge is out of $O_{j-1}$.
Similar to the proof of \textbf{claim$_{II}$}, each node $O_k$ where $0\leq k\leq j-1$ must be adjacent to $O_{j+1}$ and the edge is out of $O_k$ in $\mathcal{M}$.
Then, $X$ and $O_{j+1}$ are adjacent and the edge is out of $X$ in $\mathcal{M}$.
This edge has to be visible in $\mathcal{M}$ for otherwise we violate our choice of $p^*$.
Consider the shortest path into $X$ consistent with the graphical condition for visibility that makes edge $X\rightarrow O_{j+1}$ visible in $\mathcal{M}$.
We refer to the path as $p^v$ and denote the nodes along $p^v$ as $\langle C_m,\dots C_1\rangle$ where $m\geq 1$.
Note that $m=1$ when the visibility is due to a single edge into $X$ ($C_1*\!\!\rightarrow X\rightarrow O_{j+1}$) and $C_1$ is not adjacent to $O_{j+1}$.

Let $p'$ denote the concatenated path of $p^v$ and the subpath of $p^*$ $\langle O_0=X,\dots,O_{j+1}\rangle$.
The following two points hold:

\begin{enumerate}
\item There exist at least one collider path between $C_m$ and $O_{j+1}$ over a subsequence of the non-endpoint nodes along $p'$.
Note that all the non-endpoint nodes along $p'$ are colliders in $\mathcal{M}$ except for $\langle C_1,X,O_1\rangle$ where the edge between $X$ and $O_1$ can be directed out of $X$. 
If the edge between $X$ and $O_1$ is bi-directed, then we are done as $p'$ is a collider path between $C_m$ and $O_{j+1}$ in $\mathcal{M}$.
If the edge is directed ($X\rightarrow O_1$) in $\mathcal{M}$, we prove by induction that $O_1$ is the child of every node along $p^v$ starting with $C_1$ until $O_1$ is connected with a bi-directed edge to some $C_i$ in $\mathcal{M}$.
In the base case, the edge between $C_1$ and $X$ is into $X$ so $C_1$ and $O_1$ must be adjacent for otherwise $X\rightarrow O_1$ is visible and this violates our choice of $p^*$ where none of the edges are visible.
The edge between $C_1$ and $O_1$ can't be out of $O_1$ for this violates the ancestral property of $\mathcal{M}$ due to $X\rightarrow O_1\rightarrow C_1*\!\!\rightarrow X$.
If the edge is bi-directed, then we are done.
Otherwise, the edge is out of $C_1$ and we continue with the induction step.
In the induction step, we consider node $C_i$ and assume that all the nodes $C_j$ where $1\leq j<i\leq m$ are parents of $O_1$.
This creates a collider path between $C_i$ and $X$ that is into $X$ and each collider along the path is a parent of $O_1$ hence $X\rightarrow O_1$ is visible in $\mathcal{M}$.
Thus, $C_i$ must be adjacent to $O_1$ and the edge can't be out of $O_1$ as this violates the ancestral property due to $C_{i-1}\rightarrow O_1\rightarrow C_i*\!\!\rightarrow C_{i-1}$.
Hence, the edge has to be either bi-directed or out of $C_i$.
This concludes the proof.
\item Every collider path between $C_m$ and $O_{j+1}$ over a subsequence of the non-endpoint nodes along $p'$ must go through $O_j$.
The reason is that $O_{j+1}$ is a child of each non-endpoint node along $p'$ except for $O_j$ and it is not adjacent to $C_m$ due to the visibility of edge $X\rightarrow O_{j+1}$.
$O_j$ is the only node among the nodes in $p'$ such that $O_{j+1}$ is connected to and the edge is into $O_j$ in $\mathcal{M}$.
Hence, the second point is valid as well.
\end{enumerate}

By the above two points, we choose the shortest collider path in $\mathcal{M}$ between $C_m$ and $O_{j+1}$ over any subsequence of the nodes along $p'$.
By lemma II, this is a definite status path in $\mathcal{P}$, and the edge between $O_{j+1}$ and $O_j$ is into $O_j$.

If the edge between $O_{j-1}$ and $O_j$ has a circle incident on $O_j$ in $\mathcal{P}$, then the edge between $O_{j-1}$ and $O_{j+1}$ has an arrowhead incident on $O_{j-1}$ in $\mathcal{P}$ (Lemma~\ref{lem:cppag}).
However, this is not possible as the edge between $O_{j-1}$ and $O_{j+1}$ is out of $O_{j-1}$ in $\mathcal{M}$ according to the assumption in the base case of the proof of \textbf{claim}$_I$.
Since $\mathcal{P}$ is the PAG representing the equivalence class of $\mathcal{M}$, then $\mathcal{P}$ can't have an arrowhead incident on $O_{j-1}$ from $O_{j+1}$ as this orientation is not invariant in all the MAGs in the equivalence class.
Hence, the edge between $O_{j-1}$ and $O_j$ can't have a circle incident on $O_j$ and the edge will be into $O_j$ in $\mathcal{P}$.
Having $O_j$ a definite collider along $\langle O_{j-1},O_j,O_{j+1}\rangle$ contradicts our assumption in the base case that $O_j$ is the first node that is not of definite status along $p^*$ in $\mathcal{P}$.
Hence, the initial assumption that the edge between $O_{j-1}$ and $O_{j+1}$ is out of $O_{j-1}$ in $\mathcal{M}$ is invalid and the edge must be out of $O_{j+1}$.

In the induction step, we apply the exact same argument as that applied in the induction step of the proof of \textbf{claim$_{II}$}.
We omit the proof to avoid redundancy.
This concludes the proof of claim$_{I}$.
Next, we prove the following claim which is symmetric to \textbf{claim$_I$}.

\begin{quote}[\textbf{claim$_I^*$}: ]
For every $1\leq j\leq n-1$, if $O_j$ is not of a definite status on $p^*$ in $\mathcal{P}$, then $O_{j-1}$ is a parent of $O_{j+1}$ in $\mathcal{M}$.
\end{quote}

Again, the proof of \textbf{claim$_I^*$} is exactly the same as the proof of \textbf{claim$_I$} with the difference of starting the induction with the first node that is not of definite status along $p^*$ and is closest to $Y$ instead of $X$.
However, having both claims valid is contradicting as long as there exist at least one non-definite status node along $p^*$ in $\mathcal{P}$.
Hence, path $p^*$ is of definite status and any directed edge along the path of not visible. 
This concludes our proof for the main lemma.
\end{proof}

\subsection{Theorem \ref{th:bucketidpag}}

\begin{proof}[Proof of Theorem \ref{th:bucketidpag}]
\textbf{(if) }
Let $\mathcal{D}$ be any DAG in the equivalence class represented by $\mathcal{P}$, $\mathcal{D}_\mathbf{T}$ be the induced subgraph over $\mathbf{T}$, and $S'$ be the smallest composite c-component containing $\mathbf{X}$ in $\mathcal{D}_\mathbf{T}$.
We show that $\mathbf{X}$ is a descendant set in $\mathcal{D}_{S'}$.
Suppose otherwise for the sake of contradiction.
Then, there is a node $C\in S'\backslash\mathbf{X}$ such that $C$ is a child of $X_i$ and is in the same c-component with $X_j$, where $X_i,X_j\in\mathbf{X}$ and possibly $i=j$.
By Prop.~\ref{prop:pccompsubpag}, $X_j$ is in the same pc-component with $C$ in $\mathcal{P}_\mathbf{T}$.
Let $T_i$ be the node closest to $X_j$ along the collider path in $\mathcal{P}_\mathbf{T}$ between $X_j$ and $C$ consistent with Def.~\ref{def:pccomp}.
If the edge between $X_j$ and $T_i$ in $\mathcal{P}_\mathbf{T}$ is not into $X_j$, then $X_j$ is in the same pc-component with a possible child as the edge is not visible.
This violates the criterion stated in the theorem.
Otherwise, the edge is $X_j\leftrightarrow T_i$ and there exist a bi-directed edge between $T_i$ and every node in $\mathbf{X}$ (which follows from Lemma~\ref{lem:cpsubpag}).
Hence, $X_i$ is in the same pc-component with a possible child $C$ in $\mathcal{P}_\mathbf{T}$ (Prop.~\ref{prop:ancsubpag}), and the criterion stated in the theorem is violated again.
Therefore, $\mathbf{X}$ is a descendant set in $\mathcal{D}_{S'}$ and $Q[\mathbf{T}\setminus\mathbf{X}]$ is identifiable from $Q[\mathbf{T}]$ by Lemma~\ref{lem:subsetiddag}.
It remains to show that Eq.~\ref{eq:bucketidpag} is equivalent to Eq.~\ref{eq:subsetiddag} for $\mathcal{D}$.
Eq.~\ref{eq:bucketidpag} differs from Eq.~\ref{eq:subsetiddag} by using:
\begin{enumerate}
\item \label{enum:1}product of conditional terms instead of $Q[S^\mathbf{X}]$,
\item \label{enum:2}conditional terms over buckets instead of single variables, and
\item \label{enum:3}dc-component instead of c-component.
\end{enumerate}

In what follows, we address those differences.
\vspace{-1em}
\paragraph{(\ref{enum:1})}
Consider Eq.~\ref{eq:qhidag} which computes $Q[\mathbf{H}_j]$ from $Q[\mathbf{H}]$.
Each fraction $\frac{Q[H^{(i)}]}{Q[H^{(i-1)}]}$ for node $V_{h_i}$ is nothing but the conditional probability $P_{\mathbf{v}\setminus\mathbf{h}}(V_{h_i}|V^{h_{i-1}})$, where $Q[\mathbf{H}]$ is identifiable and given by $P_{\mathbf{v}\setminus\mathbf{h}}$.
Therefore, the product of conditional terms in Eq.~\ref{eq:bucketidpag} substitutes $Q[S^\mathbf{X}]$ in Eq. 2 whenever $S^\mathbf{X}$ corresponds to the composite c-component containing $\mathbf{X}$ in $\mathcal{D}$.
Whether the latter is true or not is addressed in point~\ref{enum:3}.
\vspace{-1em}
\paragraph{(\ref{enum:2})}
If some node in bucket $\mathbf{B}$ is in the dc-component of $X_i\in\mathbf{X}$, then every node in $\mathbf{B}$ is in the same dc-component with each node in $\mathbf{X}$ (Lemma~\ref{lem:332}).
It follows that the dc-component of $\mathbf{X}$ is a union of one or more buckets in $\mathcal{P}_\mathbf{T}$.
For any full topological order over $\mathbf{T}$ that is consistent with the partial order used in Eq.~\ref{eq:bucketidpag}, the nodes within a bucket will be consecutive.
Hence, the corresponding conditional terms can be jointly expressed by $P_{\mathbf{v}\setminus\mathbf{t}}(\mathbf{B_i}|\mathbf{B^{(i-1)}})$.
\vspace{-1em}
\paragraph{(\ref{enum:3})}
The pc-component of $\mathbf{X}$ in $\mathcal{P}_\mathbf{T}$ subsumes the composite c-component containing $\mathbf{X}$ in $\mathcal{D}_\mathbf{T}$ (Prop.~\ref{prop:pccompsubpag}).
In Eq.~\ref{eq:bucketidpag}, we exclude the nodes that are in the pc-component, but are not in the dc-component of $\mathbf{X}$.
In $\mathcal{P}_\mathbf{T}$, let $C$ be one such node in bucket $\mathbf{B_i}$ that is in the pc-component, but not the dc-component, of $\mathbf{X}$.
It follows that there is no bi-directed path between $\mathbf{X}$ and $\mathbf{B_i}$ and no node in $\mathbf{B_i}$ is in the dc-component of $\mathbf{X}$.
If $\mathbf{B_i}$ comes before $\mathbf{X}$ in the partial order, then the conditional term for $C$ in Eq.~\ref{eq:subsetiddag} doesn't condition on $\mathbf{X}$ and the term can be pushed behind the summation over $\mathbf{X}$ and cancels out with the corresponding term in the numerator.
Otherwise, consider any proper definite status path between $\mathbf{X}$ and $\mathbf{B_i}$.
One of the following properties must be true:
\begin{enumerate}
\item path contains at least one definite non-collider, or
\item path is not into $\mathbf{B_i}$, or
\item path is not into $\mathbf{X}$.
\end{enumerate}

Consider a proper definite status path between $\mathbf{X}$ and $\mathbf{B_i}$ where the first two properties don't hold, i.e. $X_i*\!\!\rightarrow Y\xdashleftrightarrow{\hspace{3em}} T_i\in\mathbf{B_i}$.
The edge between $X_i$ and $Y$ must be visible, otherwise $X_i$ is in the same pc-component with a non-intervention child ($Y$).
So, we have $Y$ in the dc-component of $T_i$, and consequently in the dc-component of every node in $\mathbf{B_i}$.
\achange{
Also, note that the first edge along the collider path between $\mathbf{X}$ and $C$ consistent with Def.~\ref{def:pccomp} is into $\mathbf{X}$, otherwise we violate the theorem condition.
It follows that in $\mathcal{P}_\mathbf{T}$, $C$ is in the dc-component of $Y$ and $C$ is also in the pc-component of $X_i$ while $Y$ is a child of $X_i$.
Hence, we can construct a DAG $\mathcal{D}'$ in the equivalence class of $\mathcal{P}$ where $X_i$ and $Y$ are in the same c-component while $Y$ is a child of $X_i$
%(Lemmas~\ref{lem:PAGMAGcomp} and~\ref{lem:MAGDAGcomp}).
(Lemmas~\ref{lem:PAGMAGinvisibleedge} and~\ref{lem:MAGDAGinvisibleedge}).}
In the subgraph $\mathcal{D}'_\mathbf{T}$, $X_i$ remains in the same c-component with $Y$, hence $X_i$ will be in the pc-component of $Y$ (Lemma~\ref{prop:pccompsubpag}) and this violates the criterion of the proposition.
Therefore, every proper definite status path between $\mathbf{X}$ and $\mathbf{B_i}$ in $\mathcal{P}_\mathbf{T}$ has one of the first two properties true.

Also, no node in $\mathbf{B_i}$ is adjacent to a node in $\mathbf{X}$ in $\mathcal{P}_\mathbf{T}$.
Suppose for contradiction that the latter is not true.
So the edge between the two buckets must be bi-directed or possibly out of $\mathbf{X}$ and into $\mathbf{B_i}$ ($X_i*\!\!\rightarrow T_i\in\mathbf{B_i}$) as $\mathbf{B_i}$ comes after $\mathbf{X}$ in the partial order.
The first case is not possible as $\mathbf{B_i}$ would be in the same dc-component as $\mathbf{X}$.
In the second case, we have a possibly directed edge in $\mathcal{P}_\mathbf{T}$ between $X_i$ and every node in $\mathbf{B_i}$ including $C$ (Lemma~\ref{lem:332}).
So, $X_i$ will be in the same pc-component with a possible child ($C$) which contradicts the criterion in the current proposition.
By Lemmas~\ref{lem:bindep}, \ref{lem:defpathsubpag}, and~\ref{lem:connpathsubmag}, we have $(\mathbf{B_i}\independent\mathbf{X}|\mathbf{B^{(i-1)}}\setminus\mathbf{X})$ in $\mathcal{D}_\mathbf{T}$.
This implies that the conditional term of $C$ is independent of $\mathbf{X}$, and even if it was included in $S^\mathbf{X}$, the expression can be simplified to the one in Eq.~\ref{eq:bucketidpag}.

This concludes the proof for when $\mathbf{T}=\mathbf{V}$ as $\mathcal{P}_\mathbf{T}$ will be the full PAG.
A bi-directed edge in a PAG implies that the two nodes are in the same c-component in every DAG in the equivalence class, hence the dc-component of $\mathbf{X}$ in $\mathcal{P}$ is part of the composite c-component of $\mathbf{X}$ in $\mathcal{D}$.
However, $\mathcal{P}_\mathbf{T}$ preserves the causal relations between the nodes in $\mathcal{D}_\mathbf{T}$, but not necessarily the spurious ones (Prop.~\ref{prop:ancsubpag}).
Hence, it is not necessarily true that $S^\mathbf{X}$ is a subset of the composite c-component of $\mathbf{X}$ in $\mathcal{D}_\mathbf{T}$.

Let $T_i\in\mathbf{B_i}\subset S^\mathbf{X}$ be a node in $\mathcal{D}_\mathbf{T}$ which is not in the composite c-component of $\mathbf{X}$, let $\mathcal{M}$ be the MAG corresponding to $\mathcal{D}_\mathbf{T}$, and consider a full topological order over $\mathcal{M}$ that is consistent with the partial order in Th.~\ref{th:bucketidpag}.
If $T_i$ comes before $\mathbf{X}$ in the full order, then $\mathbf{B_i}$ comes before $\mathbf{X}$ in the partial order over $\mathcal{P}_\mathbf{T}$ and the conditional term in Eq.~\ref{eq:bucketidpag} doesn't condition on $\mathbf{X}$.
Hence, Eq.~\ref{eq:bucketidpag} is valid for $\mathcal{D}_\mathbf{T}$ as we can use the full order to decompose the conditional term of $\mathbf{B_i}$, then simplify the expression by canceling the conditional term for $T_i$ with the corresponding one in the denominator.
The other option is when $T_i$ comes after $\mathbf{X}$ in the full order and consequently the partial order over $\mathcal{P}_\mathbf{T}$.
Since $T_i$ is not in the c-component of any node in $\mathbf{X}$, then there is no bi-directed path between $T_i$ and $\mathbf{X}$ in $\mathcal{M}$ and one of the following is true for any proper path between them:
\begin{enumerate}
\item path contains at least one non-collider, or
\item path is out of $T_i$, or
\item path is out of $\mathbf{X}$.
\end{enumerate}

Consider a proper path between $X_i\in\mathbf{X}$ and $T_i$ in $\mathcal{M}$ where the first two properties don't hold, i.e. $X_i\rightarrow Y\xdashleftrightarrow{\hspace{3em}} T_i$.
Since $Y$ and $T_i$ share a bi-directed path in $\mathcal{M}$, then $Y$ and $T_i$ are in the same c-component in $\mathcal{D}_\mathbf{T}$.
But, $X_i$ and $T_i\in S^{\mathbf{X}}$ are in the same dc-component in $\mathcal{P}_\mathbf{T}$, and consequently $\mathcal{P}$.
Hence, $X_i$ and $Y$ are in the same c-component in $\mathcal{D}$.
It follows that we can construct a DAG $\mathcal{D}'$ in the equivalence class of $\mathcal{P}$ such that $X_i$ and $Y$ are in the same c-component in $\mathcal{D}'_\mathbf{T}$ while keeping $Y$ a child of $X_i$.
Hence, $X_i$ will be in the same pc-component with a possible child $Y$ in $\mathcal{P}_\mathbf{T}$ (Props.~\ref{prop:ancsubpag} and \ref{prop:pccompsubpag}).
The latter violates the criterion of the theorem at hand, hence such a path cannot exist in $\mathcal{M}$ and every proper path between $\mathbf{X}$ and $T_i$ must have one of the first two properties true.

Also, $T_i$ is not adjacent to any node in $\mathbf{X}$ in $\mathcal{M}$.
Suppose for contradiction that the latter is not true.
If the edge is bi-directed, this contradicts the assumption that $T_i$ is not in the same c-component of any node in set $\mathbf{X}$ in $\mathcal{D}_\mathbf{T}$.
If the edge is directed, it must be out of $\mathbf{X}$ ($X_i\rightarrow T_i$) as $T_i$ comes after $\mathbf{X}$ in the partial order.
$\mathcal{P}_\mathbf{T}$ preserves the ancestral relations, so $T_i$ must be a possible child of $X_i$ while being in the same dc-component as $\mathbf{X}$ in $\mathcal{P}_\mathbf{T}$.
This violates the criterion of the proposition, so $T_i$ is not adjacent to any node in $\mathbf{X}$ in $\mathcal{M}$.
By an argument similar to that of Lemma~\ref{lem:bindep}, we have $(T_i\independent\mathbf{X}|\mathbf{T^{(i-1)}}\setminus\mathbf{X})$ in $\mathcal{M}$ and consequently in $\mathcal{D}_\mathbf{T}$.
This implies that the conditional term of $T_i$ under the full order is independent of $\mathbf{X}$ in $\mathcal{D}_\mathbf{T}$, and even if it was included in $S^\mathbf{X}$, the expression specific to $\mathcal{D}_\mathbf{T}$ can be rewritten as the one in Eq.~\ref{eq:bucketidpag}.
Therefore, the expression is unanimous and this concludes the proof.

\textbf{(only if) }
Whenever the criterion fails, we show that we can construct a DAG in the equivalence class of $\mathcal{P}$ such that the effect is not identifiable.
By Def.~\ref{def:idpag}, the effect is not identifiable in $\mathcal{P}$.
If the criterion is not satisfied, then some node $X_i\in\mathbf{X}$ is in the pc-component with a non-intervention possible child $C$ in $\mathcal{P}_\mathbf{T}$.
The edge between $X_i$ and $C$ is $X_i*\!\!\rightarrow C$ as $C$ is outside the bucket of $X_i$.
If the edge is not visible in $\mathcal{P}_\mathbf{T}$, then this edge is not visible in $\mathcal{P}$ (Lemma~\ref{lem:subpagvis}).
Hence, we can construct a DAG $\mathcal{D}$ in the equivalence class of $\mathcal{P}$ where $C$ is a child of $X_i$ and the two nodes share a latent variable (Lemmas~\ref{lem:PAGMAGinvisibleedge} and \ref{lem:MAGDAGinvisibleedge}).
The pair of sets $\mathbf{F}=\{X_i,C\}$ and $\mathbf{F}'=\{C\}$ form a hedge for $Q[\mathbf{T}\setminus\mathbf{X}]$ and the effect is not identifiable in $\mathcal{D}$ \citep[Theorem 4]{shpitser2006identification}.

Otherwise, the edge $X_i\rightarrow C$ is visible in $\mathcal{P}_\mathbf{T}$.
Then, there is a collider path between $X_i$ and $C$ consistent with Def.~\ref{def:pccomp} such that the two nodes are in the same pc-component.
Let $p\!\!=\!\!\langle X_i\!\!=\!\!T_0,T_1,\dots,T_m\!\!=\!\!C\rangle$ denote the shortest such path in $\mathcal{P}_\mathbf{T}$.
If the edge between $X_i$ and $T_1$ is not into $X_i$, then $T_1$ is a possible child of $X_i$ and the proof follows as in the previous case.
Otherwise, we have $X_i\leftrightarrow T_1$.
In this case, $X_i$ is the only node along the path that belongs to $\mathbf{X}$.
Suppose for contradiction that there is another node along the path which belongs to $\mathbf{X}$ and let $T_i$ be one such node that is closest to $X_i$.
We have $T_i\leftrightarrow T_{i+1}$ along the path and $T_{i+1}\neq C$, otherwise we $T_i\leftarrow\!\!*$ with a possibly directed path from $T_i$ to $C$ through $X_i$ which is not possible (Lemma~\ref{lem:nocycle}).
Then, there is a bi-directed edge between $T_{i+1}$ and every node in $\mathbf{X}$ (Lemma~\ref{lem:332}).
This creates a shorter path than the initial one chosen composed of the sequence $\langle X_i,T_{i+1},\dots,C\rangle$ which is a contradiction.
In $\mathcal{P}$, path $p$ is present with $X_i\rightarrow C$ visible.
Hence, we can construct a DAG $\mathcal{D}$ in the equivalence class of $\mathcal{P}$ such that $C$ is a child of $X_i$ and both are in the same c-component through a sequence of bi-directed edges along $\langle X_i,T_1,\dots,C\rangle$ (Lemmas~\ref{lem:PAGMAGinvisibleedge} and \ref{lem:MAGDAGinvisibleedge}).
The pair of sets $\mathbf{F}=\{X_i,T_1,\dots,C\}$ and $\mathbf{F}'=\{T_1,\dots,C\}$ form a hedge for $Q[\mathbf{T}\setminus\mathbf{X}]$ and the effect is not identifiable in $\mathcal{D}$.
This concludes the proof.
\end{proof}

\begin{comment}
\begin{lemma}
Let $\mathcal{P}$ be a PAG over a set of variables $\mathbf{V}$, and $A$ and $B$ be two nodes that are in the same pc-component in $\mathcal{P}$.
There is a MAG in the equivalence class of $\mathcal{P}$ where $A$ and $B$ are in the same pc-component if $A$ and $B$ in $\mathcal{P}$ are adjacent or in different buckets (i.e. no circle path between them).
\label{lem:PAGMAGcomp}
\end{lemma}

\begin{proof}
Under the conditions of the lemma, we have the following options for $A$ and $B$ to be in the same pc-component:

\begin{enumerate}
\item $A$ and $B$ are adjacent and the edge not fully oriented, bi-directed, or directed and not visible in $\mathcal{P}$: If the edge is bi-directed in $\mathcal{P}$, then it is bi-directed in every MAG $\mathcal{M}$. Otherwise, the edge is oriented in some MAG into an invisible directed edge by lemma~\ref{lem:PAGMAGinvisibleedge}.
\item $A$ and $B$ are in different circle components of PAG $\mathcal{P}$ (different buckets), they share a collider path ($A*\!\!\rightarrow O_1\xdashleftrightarrow{\hspace{2.5em}} O_n\leftarrow\!\! *B$), and any directed edge is not visible.
By lemma~\ref{lem:nonewarrowsX}, we can construct a MAG $\mathcal{M}$ in the equivalence class of $\mathcal{P}$ such that we have no new edges into $A$ nor into $B$.
This extension to the lemma is possible since $A$ and $B$ correspond to two separate circle components in $\mathcal{P}$ according to the condition in the lemma.
Hence, the orientations can be done independently in each circle component.
Therefore, both edges $A\rightarrow O_1$ and $O_n\leftarrow B$ are invisible in $\mathcal{M}$ by lemma~\ref{lem:PAGMAGinvisibleedge}.
The latter is correct as the same argument in the proof of lemma~\ref{lem:PAGMAGinvisibleedge} can be made for both edges simultaneously.
Thus, we have a collider path between $A$ and $B$ in MAG $\mathcal{M}$ ($A\rightarrow O_1\xdashleftrightarrow{\hspace{2.5em}} O_n\leftarrow B$) and the first and last edges are not visible.
\end{enumerate}
\end{proof}

\begin{lemma}
Let $\mathcal{M}$ be any MAG over a set of variables $\mathbf{V}$.
If $A$ and $B$ are in the same pc-component in $\mathcal{M}$, then there is a DAG in the equivalence class of $\mathcal{M}$ where $A$ and $B$ are in the same c-component.
\label{lem:MAGDAGcomp}
\end{lemma}

\begin{proof}
If $A$ and $B$ are in the same pc-component in MAG $\mathcal{M}$, then one of the following must be true:
\begin{enumerate}
\item $A$ and $B$ are adjacent in $\mathcal{M}$ and the edge is not visible: A DAG is constructed according to lemma~\ref{lem:MAGDAGinvisibleedge} where $A$ and $B$ share a latent parent $L_{AB}$.
\item A collider path exists between $A$ and $B$ where no directed edge is visible ($A*\!\!\rightarrow O_1\xdashleftrightarrow{\hspace{2.5em}} O_n\leftarrow\!\! *B$): If $A*\!\!\rightarrow O_1$ or $O_n\leftarrow\!\! *B$ is bi-directed in $\mathcal{M}$, then the construction in lemma~\ref{lem:MAGDAGinvisibleedge} creates a DAG where $A$ and $B$ share a bi-directed path and hence are in the same c-component.

The other case is when both $A*\!\!\rightarrow O_1$ and $O_n\leftarrow\!\! *B$ are directed invisible edges.
If $A$ and $B$ share a bi-directed path in $\mathcal{M}$, then the previous construction puts $A$ and $B$ in the same c-component in a DAG $\mathcal{G}$.
Otherwise, the conditions of lemma~\ref{lem:MAGDAG2invisibleedge} are satisfied and we construct a DAG $\mathcal{G}$ in the equivalence class of $\mathcal{M}$ where $A\rightarrow O_1$ and $O_n\leftarrow B$ are confounded simultaneously. Hence, $A$ and $B$ are in the same c-component in $\mathcal{G}$.
\end{enumerate}
\end{proof}

\begin{lemma}
Let $\mathcal{M}$ be any MAG over a set of variables $\mathbf{V}$, and $A\rightarrow B$ and $C\rightarrow D$ be any two invisible directed edges in $\mathcal{M}$ such that $A\neq C$.
If there is no bi-directed path between $A$ and $C$ in $\mathcal{M}$, then there is a DAG whose MAG is $\mathcal{M}$ in which $A$ and $B$ share a latent parent and $C$ and $D$ share another latent parent simultaneously.
\label{lem:MAGDAG2invisibleedge}
\end{lemma}

\begin{proof}
Under the condition in the lemma, construct a DAG $\mathcal{G}$ from $\mathcal{M}$ using the following steps:

\begin{enumerate}
\item Leave every directed edge in $\mathcal{M}$ as it is.
\item Replace every bi-directed edge $U\leftrightarrow W$ in $\mathcal{M}$ with a latent variable $L_{UW}$ between $U$ and $W$.
\item Introduce two additional latent variables: $L_{AB}$ between $A$ and $B$ and $L_{CD}$ between $C$ and $D$.
\end{enumerate}

In order to prove the lemma, we need to show that $\mathcal{M}_{\mathcal{G}}=\mathcal{M}$ where $\mathcal{M}_{\mathcal{G}}$ is the MAG corresponding to DAG $\mathcal{G}$.
Hence, we have the following exhaustive options given any pair of variables $X$ and $Y$:

\begin{enumerate}
\item $X\rightarrow Y$ in $\mathcal{M}$: DAG $\mathcal{G}$ retains the same directed edges in $\mathcal{M}$, so the same edge is present in $\mathcal{M}_{\mathcal{G}}$.
\item $X\leftarrow Y$ in $\mathcal{M}$: Same as the previous case.
\item $X\leftrightarrow Y$ in $\mathcal{M}$: $\mathcal{G}$ replaces every bi-directed edge in $\mathcal{M}$ with a latent variable which in turn is an inducing path between $X$ and $Y$ in $\mathcal{G}$. Since the construction of $\mathcal{G}$ doesn't introduce any new ancestral relations between variables other than the ones already present in $\mathcal{M}$, then $X\leftrightarrow Y$ is present in $\mathcal{M}_{\mathcal{G}}$.
\item $X$ and $Y$ are not adjacent in $\mathcal{M}$: In this case, we need to show that there is no inducing path between $X$ and $Y$ in $\mathcal{G}$. In what follows, we prove this result using contradiction.
\end{enumerate}

Suppose that there is an inducing path between $X$ and $Y$ in $\mathcal{G}$ while they are not adjacent in $\mathcal{M}$.
Let $p$ be such a path with the smallest number of observed variables in $\mathcal{G}$ and let $\langle X,O_1,\dots,O_n,Y\rangle$ denote the sequence of observed nodes along the path.
Since the construction of $\mathcal{G}$ doesn't introduce new ancestral relations than the ones in $\mathcal{M}$, then each node $O_i$ must be an ancestor of $X$ or $Y$ in $\mathcal{M}$ as well as in $\mathcal{G}$.
If a maximum of one of the edges $A\rightarrow B$ and $C\rightarrow D$ is along the inducing path $p$, then the proof by contradiction follows exactly as that in \citep[Lemma 5.1.2]{zhang2006causal}.

It remains to consider the case where both edges are along the inducing path $p$.
The condition in the lemma states that $A\neq C$ and there is no collider path between $A$ and $C$ in $\mathcal{M}$.
So by the construction of $\mathcal{G}$, we can't have $B\leftarrow A\xdashleftrightarrow{\hspace{2.5em}} C\rightarrow D$ as a sub-path of $p$ with zero or more intermediate observed variables.
Hence, both edges ($A\rightarrow B$ and $C\rightarrow D$) can exist along $p$ simultaneously if we have one of the following as sub-path of $p$:
\begin{enumerate}
\item $A\rightarrow B\xdashleftrightarrow{\hspace{2.5em}} D\leftarrow C$: Without loss of generality, suppose that $X$ is closest to $A$ along the path and $Y$ is closest to $C$.
If $X=A$ and $Y=C$, then both $A\rightarrow B$ and $C\rightarrow D$ are into $O_1=B$ and $O_n=D$ in $\mathcal{M}$, respectively.
As for the intermediate edges along $p$, they correspond to latent variables $L_{O_iO_{i+1}}$ for $1<i<n-1$.
Those latent variables correspond to bi-directed edges in $\mathcal{M}$ by construction of $\mathcal{G}$.
Therefore, an inducing path between $X$ and $Y$ is present in $\mathcal{M}$.
This is not possible as it contradicts with the maximality property of a MAG.

If $X\neq A$ or $Y\neq C$, at least one of the two edges is not the first along $p$.
Without loss of generality, suppose that $A\rightarrow B$ is one such edge.
The edge between $X$ and $O_1$ in $\mathcal{M}$ must be into $O_1$ as it is into $O_1$ in $\mathcal{G}$.
Also, every intermediate edge between $O_1$ and $O_i=A$ in $\mathcal{M}$ must be bi-directed as it corresponds to a latent variable in $\mathcal{G}$.
We argue by induction that every node $O_j$ $j<i$ is a parent of $B$ in $\mathcal{M}$.
In the base case, $O_{i-1}$ is adjacent to $B$ or else $A\rightarrow B$ is visible.
The edge between $O_{i-1}$ and $B$ is not out of $B$ as it violates the ancestral property of $\mathcal{M}$ due to $A\rightarrow B\rightarrow O_{i-1}$ and $O_{i-1}\leftrightarrow O_i$.
Also, the edge is not bi-directed as this would lead to an inducing path in $\mathcal{G}$ shorter than $p$. In the inductive step, assume all the nodes starting with $O_{i-1}$ till $O_j$ are parents of $B$. Then, $O_{j+1}$ must be adjacent to $B$, else $A\rightarrow B$ is visible.
Also, the edge has to be out of $O_{j+1}$ for the same reasons as before.
This implies that $X$ is adjacent to $B$ and the edge is into $B$ in $\mathcal{M}$.
Again, we have an inducing path between $X$ and $Y$ in $\mathcal{G}$ that has fewer number of observed variables than $p$ which is a contradiction.
\item $A\rightarrow B\xdashleftrightarrow{\hspace{2.5em}} C\rightarrow D$: Again, without loss of generality, suppose that $X$ is closest to $A$ along the path and $Y$ is closest to $D$.
If $X\neq A$, we can use the same proof by induction as before to show that every node along $p$ starting with $X$ until $A$ is a parent of $B$ in $\mathcal{M}$.
Hence, we have an inducing path in $\mathcal{G}$ with fewer observed variables than $p$ which is a contradiction.

If $X=A$, then we have a collider path into $C$ starting with $X=A$ in $\mathcal{M}$.
Again, every node along this path is a parent of $D$ by the induction earlier.
Hence, $X$ is a parent of $D$ in $\mathcal{M}$ and we have a shorter inducing path than $p$ which is a contradiction.
\item $B\leftarrow A\xdashleftrightarrow{\hspace{2.5em}} D\leftarrow C$: The argument for this case is the same as the previous case.
\end{enumerate}

The latter three cases all arrive to contradictions, thus a pair of variables that is not adjacent in $\mathcal{M}$ is not adjacent in $\mathcal{M}_{\mathcal{G}}$ as well.
Therefore, $\mathcal{M}=\mathcal{M}_{\mathcal{G}}$.
\end{proof}
\end{comment}

\achange{
\begin{lemma}
Given a PAG $\mathcal{P}$, a corresponding partial order $\mathbf{B}_1<\dots<\mathbf{B}_m$, a bucket $\mathbf{B}_i$, and $\mathbfcal{H}$ a subset of the buckets in $\mathbf{B}^{(i-1)}$.
Then, $\mathbf{B}_i$ is independent of $\mathbfcal{H}$ given $\mathbf{B}^{(i-1)}\setminus\mathbfcal{H}$, i.e. ($\mathbf{B}_i\independent\mathbfcal{H}|\mathbf{B}^{(i-1)}\setminus\mathbfcal{H})$, if:
\begin{enumerate}
\item $\nexists (v_i\in \mathbf{B}_i \wedge v_j\in\mathbfcal{H} \wedge v_i *\!\!\--*\!\!v_j)$, i.e. there is no path of size one connecting $\mathbf{B}_i$ and $\mathbfcal{H}$, and
\item Each proper definite status path between $\mathbf{B}_i$ and $\mathbfcal{H}$:
\begin{enumerate}
\item Contains at least one definite non-collider, or% not in $\mathbfcal{H}$, or
\item The path is not into $\mathbf{B}_i$.
\end{enumerate}
\end{enumerate}
\label{lem:bindep}
\end{lemma}

\begin{proof}
%Any subset of $\mathbf{B^{(i-1)}}$ refers to a subset of the buckets represented by $B^{(i-1)}$.
The first condition is necessary as it is not possible to separate two sets of nodes in a PAG if there exist $v_i\in\mathbf{B}_i$ and $v_j\in\mathbfcal{H}$ such that $v_i$ and $v_j$ are adjacent.
By \citep[Lemmas 5.1.3 and 5.1.7]{zhang2006causal}, we need to block the definite status paths between any $v_i\in\mathbf{B_i}$ and $v_j\in\mathbfcal{H}$ for $\mathbf{B_i}$ and $\mathbfcal{H}$ to be independent.
But, any definite status path between $v_i$ and $v_j$ includes one of the proper definite status paths between $\mathbf{B_i}$ and $\mathbfcal{H}$ as a subpath.
Hence, we only consider blocking the proper definite status paths between $\mathbf{B_i}$ and $\mathbfcal{H}$ since this will be sufficient to block all the definite status paths between any $v_i\in\mathbf{B_i}$ and $v_j\in\mathbfcal{H}$.
For simplicity, we assume that a path starts from $\mathbf{B_i}$ to $\mathbfcal{H}$.
%
Consider any proper definite status path between $\mathbf{B_i}$ and $\mathbfcal{H}$; $p=\langle O_1,\dots,O_n\rangle$ where $n>2$, $O_1\in\mathbf{ B_i}$, $O_n\in\mathbfcal{H}$.%, and $O_2,\dots,O_{n_1}\notin\mathbf{B_i} \cup \mathbfcal{H}$.

\begin{enumerate}
\item The path contains at least one definite non-collider %not in $\mathbfcal{H}$ 
denoted $O_l\in\mathbf{B_k}$.
If $k<i$, then the path is blocked as $O_l\in\mathbf{B}^{(i-1)}\setminus\mathbfcal{H}$.
If $k>i$, then $O_l$ is in a bucket that comes after $\mathbf{B_i}$ in the partial order.
Without loss of generality, let $p_1=\langle O_l,\dots,O_1\rangle$ be the subpath of $p$ that is possibly out of $O_l$.
By the partial order, there must exist a collider along $p_1$, else $O_l$ is a possible ancestor of $O_1$.
The collider is not in $\mathbf{B}^{(i-1)}\setminus\mathbfcal{H}$ nor any of its possible descendants.
Hence, the collider blocks $p$.
% We show that at least one of the subpaths $p_1=\langle O_1,\dots,O_l\rangle$ and $p_2=\langle O_l,\dots,O_n\rangle$ must contain a collider and this collider is in a bucket $\mathbf{B_p}$ where $p>k>i$.
% Note that path $p$ is of definite status so each non-endpoint node along the path should be a definite collider or a definite non-collider (DNC).

% \begin{itemize}
% \item[\textbf{DNC 1}] Consider one of the edges of $O_l$ along path $p$ to be out of $O_l$. Without loss of generality, we consider the target node of the edge to be $O_{l+1}$ ($O_l \rightarrow O_{l+1}$).
% A bucket only contains circle edges, so $O_{l+1}$ can't be in the same bucket as $O_l$.
% Hence, it must be in another bucket $\mathbf{B_p}$ where $p>k$ since the edge is directed.
% \item[\textbf{DNC 2}] The DNC is such that $O_{l-1}*\!\!\--\!\!\circ O_l\circ\!\!\--\!\!*O_{l+1}$ and $O_{l-1}$ and $O_{l+1}$ are not adjacent: If at least one of the two edges has an arrowhead on the other end, then the target node would be in a bucket $\mathbf{B_p}$ where $p>k$ for a similar argument as in \textbf{DNC 1}.
% If both edges have circles on the other ends ($O_{l-1}\circ\!\!\--\!\!\circ O_l\circ\!\!\--\!\!\circ O_{l+1}$), then the three nodes reside in the same bucket.
% Only a DNC with one of the edge $\rightarrow$ or $\circ\!\!\rightarrow$ would preserve the definite status property of path $p$ and extend it to a node outside the current bucket.
% Again, that target node will be in a bucket $\mathbf{B_p}$ where $p>k$.
% \end{itemize}

% Therefore, a sequence of DNCs along path $p$ starting with $O_l$ keeps extending path $p$ within $\mathbf{B_k}$ or to buckets ahead of it relative to the PTO.
% Only a definite collider would connect the path back to $\mathbf{B_i}$ or $\mathbfcal{H}$.
% Note that the definite collider will be in a bucket $\mathbf{B_p}$ where $p>i$ and all the possible descendants of the collider will be in buckets including and after $\mathbf{B_p}$. 
% Hence, this collider blocks the path since no possible descendants is in $\mathbf{B_i}$ or $\mathbf{B^{(i-1)}}$.

\item If the path is not into $\mathbf{B_i}$, then the edge mark incident on $O_1$ is either a tail ($O_1\rightarrow O_2$) or a circle ($O_1\circ\!\!\rightarrow O_2$).
If a circle is incident on $O_1$, then the other end of the edge has to be an arrowhead ($O_1\circ\!\!\rightarrow O_2$) since a circle would put $O_2$ in the same bucket as $O_1$ and the path would not be proper anymore.
In both cases, $O_2$ is in a bucket after $\mathbf{B}_i$.
The argument for the existence of a collider after $\mathbf{B_i}$ along path $p$ follows similar to case a.
Hence, path $p$ is blocked as well.
\end{enumerate}

Therefore, the set $\mathbf{B}^{(i-1)}\setminus\mathbfcal{H}$ blocks all the proper paths between $\mathbf{B}_i$ and $\mathbfcal{H}$. 
This concludes the proof of the lemma.
\end{proof}}

\begin{lemma}
Let $\mathcal{M}$ be a MAG over $\mathbf{V}$, and $\mathcal{P}$ be the PAG of $\mathcal{M}$.
For any $X,Y\in\mathbf{A}\subseteq\mathbf{V}$ and $\mathbf{Z}\subseteq\mathbf{A}\setminus\{X,Y\}$,
if there is an m-connecting path between $X$ and $Y$ given $\mathbf{Z}$ in $\mathcal{M}_\mathbf{A}$, then there is a definite m-connecting path between $X$ and $Y$ given $\mathbf{Z}$ in $\mathcal{P}_\mathbf{A}$.
\label{lem:defpathsubpag}
\end{lemma}

\begin{proof}
Let $[\mathcal{M}]$ denote the equivalence class of $\mathcal{M}$ represented by $\mathcal{P}$, and $[\mathcal{M}]_\mathbf{A}$ denote the set of subgraphs over $\mathbf{A}$ of every MAG in $[\mathcal{M}]$.
Every subgraph of a MAG is a MAG as well, so $\mathcal{M}_\mathbf{A}$ is a MAG.
Let $\mathcal{P}_{[\mathcal{M}_\mathbf{A}]}$ be the PAG corresponding to $[\mathcal{M}_\mathbf{A}]$, the equivalence class of $\mathcal{M}_\mathbf{A}$.
We have the following correspondence between $\mathcal{P}_{[\mathcal{M}_\mathbf{A}]}$ and $\mathcal{P}_\mathbf{A}$:
\begin{enumerate}
\item $\mathcal{P}_{[\mathcal{M}_\mathbf{A}]}$ and $\mathcal{P}_\mathbf{A}$ have the same adjacencies, since both have the same adjacencies of $\mathcal{M}_\mathbf{A}$.
\item $\mathcal{P}_\mathbf{A}$ subsumes the edge marks in $\mathcal{P}_{[\mathcal{M}_\mathbf{A}]}$:
$\mathcal{P}_\mathbf{A}$ shows all the common edge marks in $[\mathcal{M}]_\mathbf{A}$ since $\mathcal{P}$ shows the common edge marks in $[\mathcal{M}]$.
Also, every MAG in $[\mathcal{M}]_\mathbf{A}$ is in the equivalence class of $\mathcal{M}_\mathbf{A}$, otherwise we would have a contradiction in the equivalence class of $\mathcal{M}$.
Hence, we have $[\mathcal{M}]_\mathbf{A}\subseteq [\mathcal{M}_\mathbf{A}]$.
Therefore, any common mark in $[\mathcal{M}_\mathbf{A}]$ must be common in $[\mathcal{M}]_\mathbf{A}$, and $\mathcal{P}_\mathbf{A}$ subsumes the edge marks in $\mathcal{P}_{[\mathcal{M}_\mathbf{A}]}$.
\end{enumerate}
If there is an m-connecting path between $X$ and $Y$ given $\mathbf{Z}$ in $\mathcal{M}_\mathbf{A}$, then there is a definite m-connecting path between $X$ and $Y$ given $\mathbf{Z}$ in $\mathcal{P}_{[\mathcal{M}_\mathbf{A}]}$.
By the above two points, the corresponding path in $\mathcal{P}_\mathbf{A}$ is also definitely m-connecting.
\end{proof}

\begin{lemma}
Let $\mathcal{D}(\mathbf{V},\mathbf{L})$ be a DAG, and $\mathcal{M}$ be the MAG of $\mathcal{D}$ over $\mathbf{V}$.
Also, let $\mathcal{M}^*$ be the MAG over $\mathcal{D}_\mathbf{A}$, $\mathbf{A}\subseteq\mathbf{V}$.
For any $X,Y\in\mathbf{A}$ and $\mathbf{Z}\subseteq\mathbf{A}\setminus\{X,Y\}$,
if there is an m-connecting path between $X$ and $Y$ given $\mathbf{Z}$ in $\mathcal{M}^*$, then there is an m-connecting path between $X$ and $Y$ given $\mathbf{Z}$ in $\mathcal{M}_\mathbf{A}$.
\label{lem:connpathsubmag}
\end{lemma}

\begin{proof}
The proof for this lemma follows that of \citep[Lemma 5.2.1]{zhang2006causal}.
To prove this result, it is sufficient to show that $\mathcal{M}_\mathbf{A}$ is Markov equivalent to a supergraph of $\mathcal{M}^*$.
Let $\mathbf{L}'$ denote the subset of $\mathbf{L}$ in $\mathcal{D}_\mathbf{A}$.
For any $X,Y\in\mathbf{A}$, if there is an inducing path between $X$ and $Y$ relative to $\mathbf{L}'$ in $\mathcal{D}_\mathbf{A}$, then this path is also present in $\mathcal{D}$.
Therefore, $X$ and $Y$ are adjacent in both $\mathcal{M}^*$ and $\mathcal{M}_\mathbf{A}$.

If the edge between $X$ and $Y$ in $\mathcal{M}^*$ is directed, then there is a directed path between $X$ and $Y$ in $\mathcal{D}_\mathbf{A}$ and consequently in $\mathcal{D}$.
Hence, the corresponding edge between $X$ and $Y$ in $\mathcal{M}_\mathbf{A}$ is directed as well.

If the edge between $X$ and $Y$ in $\mathcal{M}^*$ is bi-directed, then the corresponding edge in $\mathcal{M}_\mathbf{A}$ is either bi-directed or an invisible directed edge.
A bi-directed edge in $\mathcal{M}^*$ implies that there is an inducing path between $X$ and $Y$ relative to $\mathbf{L}'$ in $\mathcal{D}_\mathbf{A}$ that is into both $X$ and $Y$, and consequently that path between $X$ and $Y$ is present in $\mathcal{D}$ as well.
If the corresponding edge in $\mathcal{M}_\mathbf{A}$ is directed, then it is not visible due to the previous property.
Hence, the graphical condition for visibility in \citep[Lemma 5.1.3]{zhang2006causal} is not applicable for this edge.

At this point, (1) every directed edge in $\mathcal{M}^*$ is present in $\mathcal{M}_\mathbf{A}$, and (2) every bi-directed edge in $\mathcal{M}^*$ is represented in $\mathcal{M}_\mathbf{A}$ by a bi-directed edge or an invisible directed edge.
The rest of the proof follows the same argument as that of \citep[Lemma 5.2.1]{zhang2006causal}.
Basically, we are able to transform $\mathcal{M}_\mathbf{A}$ into a supergraph of $\mathcal{M}^*$ by replacing the conflicting invisible directed edges with bi-directed edges while preserving equivalence~\citepSupp{zhang:spirtes:2005,tian:2005}.
\end{proof}

\subsection{Theorem \ref{th:idvsgac}}

\begin{proof}[Proof of Theorem \ref{th:idvsgac}]
We show that the set Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) doesn't satisfy GAC relative to ($\mathbf{X}$,$\mathbf{Y}$) in $\mathcal{P}$ (Lemma~\ref{lem:adjsuff}), whenever $\mathbf{IDP}$ fails to identify $P_\mathbf{x}(\mathbf{y})$.
First, we make the following observations whenever $\mathbf{IDP}$ fails:
\begin{enumerate}
\item $\texttt{Identify}(\mathbf{D}_i,\mathbf{V},P)$ must contain at least one intervention $X_i\in\mathbf{X}$ when the recursive call returns \texttt{Fail}.
%If the initial call doesn't include any $X_i$ in $\mathbf{S}_i$, then $\mathbf{D}_{ij}$ is an ancestral set in $\mathcal{P}_{\mathbf{S}_i}$ by construction and the routine of $\texttt{Identify}$ (Algorithm~\ref{alg:recpagrevised}) is able to identify $Q[\mathbf{D}_{ij}]$ by intervening on each bucket in $\mathbf{S}_i\setminus\mathbf{D}_{ij}$ recursively.
%A failed call to $\texttt{Identify}$ must retain at least one intervention $X_i\in\mathbf{X}$.
The reason is that all the added interventions in $\mathbf{V}\setminus\{\mathbf{D}\cup\mathbf{X}\}$ are not possible ancestors of $\mathbf{D}$ except through $\mathbf{X}$ by construction.
Hence, if $\texttt{Identify}$ intervenes on all interventions in $\mathbf{X}$, it should intervene on all the buckets in $\mathbf{V}\setminus\mathbf{D}$.
\achange{Last, $\texttt{Identify}$ doesn't fail to identify $Q[\mathbf{D}_i]$ from $Q[\mathbf{D}]$ as $\mathbf{D}_i$ is one of the cpc-components of $\mathcal{P}_\mathbf{D}$.}

\item All the nodes remaining in a failed call $\texttt{Identify}(\mathbf{C},\mathbf{T},Q[\mathbf{T}])$ are possible ancestors of $\mathbf{Y}$ in $\mathcal{P}$.
Every node in $\mathbf{T}\setminus\mathbf{C}$ is an ancestor of $\mathbf{C}$, otherwise the recursive routine wouldn't fail.
Also, all the nodes $\mathbf{D}\supseteq\mathbf{C}$ in $\mathbf{IDP}$ are ancestors of $\mathbf{Y}$ by construction.

\item \achange{Whenever $\texttt{Identify}(\mathbf{C},\mathbf{T},Q[\mathbf{T}])$ fails, there exist $X,C\in\mathbf{T}$ such that $X\in\mathbf{X}$, $C\in\mathbf{D}$ ($\mathbf{D}=\texttt{An}(\mathbf{Y})_{\mathcal{P}_{\mathbf{V}\setminus\mathbf{X}}}$) is a possible child of $X$, and $X$ is in the same pc-component with $C$.
By point 1, there exist at least one intervention $X$ when \texttt{Identify} fails.
Let $\mathbf{B}_1<\dots<\mathbf{B}_m$ be a partial order over $\mathcal{P}_{\mathbf{T}\cap\{\mathbf{V}\setminus\mathbf{D}\}}$.
If $\mathbf{B}_m$ is a strict subset of a bucket in $\mathcal{P}_\mathbf{T}$, then $X,C\in\mathbf{B}_m$ by construction of $\mathbf{D}$.
Otherwise, $\mathbf{B}_m$ is a bucket in $\mathcal{P}_\mathbf{T}$, $\mathbf{B}_m$ is in the same pc-component with a possible child, and the possible child is in $\mathbf{D}$.
}
%Also, all the possible parents of $\mathbf{C}$ must be in $\mathbf{T}\cap\mathbf{X}$ by construction, otherwise they would be included in $\mathbf{D}$.
%The claim follows due to the failing condition of $\texttt{Identify}$ in $\mathbf{IDP}$ and the absence of possibly directed cycles outside buckets in PAGs (Lemma~\ref{lem:nocycle}).
\end{enumerate}

Let $\texttt{Identify}(\mathbf{C},\mathbf{T},Q[\mathbf{T}])$ be a recursive call that throws~\texttt{Fail} for $P_{\mathbf{x}}(\mathbf{y})$.
By point 3 above, we have an intervention $X\in\mathbf{X}$ such that $X\in\mathbf{T}$, $C\in\mathbf{D}$ is a possible child of $X$, and $X$ is in the same pc-component with $C$.
If the edge between $X$ and $C$ is not a directed visible edge, then $\mathcal{P}$ is not amenable relative to ($\mathbf{X}$,$\mathbf{Y}$) (Def.~\ref{def:amenability}), and consequently no set $\mathbf{Z}$ satisfies GAC (Def.~\ref{def:gac}) relative to ($\mathbf{X}$,$\mathbf{Y}$).
Otherwise, we have a visible edge $X\rightarrow C$ and $X$ is in the same pc-component with $C$, i.e. $p=\langle X\!\!=\!\!T_0 *\!\!\rightarrow T_1 \xdashleftrightarrow{\hspace{2.5em}} T_{m-1} \leftarrow\!\!* T_m\!\!=\!\!C\rangle$ where $T_i\in\mathbf{T}$.
Let $T_i$ be the last node along $p$ starting from $T_0$ such that $T_i\in\mathbf{X}$.
Also, let $T_j$ be the first node along $p$ starting from $T_{i+1}$ such that $T_j\in\text{Forb}(\mathbf{X}$,$\mathbf{Y},\mathcal{P})\cup\mathbf{Y}$.
%, and $T_j$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{P}$.
Note that every node in $\mathbf{T}$ is in $\mathbf{X}$, $\mathbf{Y}$, Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$), or Forb($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) by point 2 above, and $C$ is consistent with the description of $T_j$ as it is in $\text{Forb(}\mathbf{X}$,$\mathbf{Y},\mathcal{P})$ by construction except for possibly not being the first.
Based on this, we have the following exhaustive options for $T_j$:
\begin{enumerate}
\item Special case: $T_i=T_0$, $T_j=T_1$, the edge between $T_i$ and $T_j$ is possibly out of $T_i$, and $T_j\in\mathbf{Y}$ or $T_j$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$.
Hence, $\mathcal{P}$ is not amenable relative to ($\mathbf{X}$,$\mathbf{Y}$) due to the invisible edge from $T_i$ to $T_j$.

\item $T_j\in\mathbf{Y}$ or $T_j$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{P}$.
Hence, every non-endpoint node along the subpath of $p$, denoted $p'=\langle T_i,\dots,T_j\rangle$, is in Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$).
If $T_j\in\mathbf{Y}$, then we have an m-connecting proper definite status non-causal path from an intervention $T_i\in\mathbf{X}$ to a node in $\mathbf{Y}$ ($T_j$).
Consequently, Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) doesn't satisfy GAC relative to $(\mathbf{X},\mathbf{Y})$ in $\mathcal{P}$.
%Otherwise, all the non-endpoint nodes along $p'$ are in Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$).
The other option is that $T_j$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$.
By definition, there is a possibly directed path from $T_j$ to $\mathbf{Y}$ that doesn't go through any node in $\mathbf{X}$, so there is an uncovered possibly directed path between them as well which doesn't go through $\mathbf{X}$ (Lemma~\ref{lem:updp}).
Hence, we can construct a MAG $\mathcal{M}$ in the equivalence class of $\mathcal{P}$ (Lemma~\ref{lem:nonewarrowsX}) such that the uncovered path is directed.
The corresponding path of $p'$ in $\mathcal{M}$ concatenated with the later directed path form an m-connecting proper non-causal path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{M}$.
By Lemma~\ref{lem:noncausalpath}, there is a proper definite status non-causal path from $\mathbf{X}$ to $\mathbf{Y}$ that is m-connecting given Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) in $\mathcal{P}$.
Therefore, Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) doesn't satisfy GAC relative to $(\mathbf{X},\mathbf{Y})$ in $\mathcal{P}$.

\item $T_j\not\in\mathbf{Y}$ and $T_j$ is not along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$, i.e. $T_j$ is a descendant of a node that lies along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{P}$.
Let $T_k$ be the last node along $p$ that has the same properties as $T_j$,
i.e. $T_k$ is a descendant of a node that lies along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{P}$, possibly $j=k$.
When $\texttt{Identify}$ fails, all nodes in $\mathbf{T}\setminus\mathbf{C}$ are possible ancestors of $\mathbf{C}$ in $\mathcal{P}_\mathbf{T}$, so every possibly directed path from $T_k$ to $\mathbf{C}$ in $\mathcal{P}_\mathbf{T}$ is blocked by some intervention in $\mathbf{X}$.
Let $X_n$ be one such intervention in $\mathbf{X}$.
By Lemma~\ref{lem:updp}, there is an uncovered possibly directed path from $T_k$ to $X_n$, denoted $p_{kn}$.
Also, let $T_p$ be the first node along $p$ starting from $T_{k+1}$ such that $T_p$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{P}$.
There exist at least one node along $p$ that is consistent with the description of $T_p$, i.e. $C$.
Again, there is an uncovered possibly directed path from $T_p$ to some $\mathbf{Y}$, denoted $p_{py}$.
At this point, we have a few important remarks:
\begin{itemize}
\item Both paths $p_{kn}$ and $p_{py}$ are included in Forb($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) as the set is a descendant set.
\item Along the subpath of $p$ between $T_k$ and $T_p$, denoted $p_{kp}$, all the non-endpoint nodes are colliders in $\mathcal{P}$ and are included in Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$)$\cup\mathbf{Y}$ due to the selection of $T_k$ and $T_p$.
\item $T_k$ and $T_p$ are not in the same circle component in $\mathcal{P}$, or else $T_k$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ as well.
\end{itemize}

Based on the above, we construct MAG $\mathcal{M}$ in the equivalence class of $\mathcal{P}$ using Lemma~\ref{lem:nonewarrowsX}.
We orient all edges possibly out of $T_k$ and $T_p$ in $\mathcal{P}$ out of them in $\mathcal{M}$, simultaneously.
The latter is possible as both nodes are in different circle components.
In $\mathcal{M}$, both paths $p_{kn}$ and $p_{py}$ are directed and don't intersect by any node, or else $T_k$ is along a proper possibly directed path from $\mathbf{X}$ to $\mathbf{Y}$ in $\mathcal{P}$ which contradicts our choice of $T_k$.
If some node along $p_{kp}$ is in $\mathbf{Y}$ ($Y$), then there is a proper non-causal path from $\mathbf{X}$ to $\mathbf{Y}$ composed of $p_{kn}$ and the subpath of $p_{kp}$ starting with $T_k$ until $Y$.
This path is m-connecting given Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) in $\mathcal{M}$.
If no node along $p_{kp}$ is in $\mathbf{Y}$, then the concatenated path composed of $p_{nk}$, $p_{kp}$, and $p_{py}$ is a proper non-causal path from $\mathbf{X}$ to $\mathbf{Y}$.
In both cases, we have a proper definite status non-causal path from $\mathbf{X}$ to $\mathbf{Y}$ that is m-connecting given Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) in $\mathcal{P}$ (Lemma~\ref{lem:noncausalpath}).
Therefore, Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) doesn't satisfy GAC relative to $(\mathbf{X},\mathbf{Y})$ in $\mathcal{P}$.
\end{enumerate}

The above cases exhaust all the options and Adjust($\mathbf{X}$,$\mathbf{Y}$,$\mathcal{P}$) doesn't satisfy GAC relative to $(\mathbf{X},\mathbf{Y})$ in $\mathcal{P}$ for every case.
This concludes the proof.
\end{proof}
